Static Inference Meets Deep Learning: A Hybrid Type Inference Approach for Python

Type inference for dynamic programming languages such as Python is an important yet challenging task. Static type inference techniques can precisely infer variables with enough static constraints but are unable to handle variables with dynamic features. Deep learning (DL) based approaches are feature-agnostic, but they cannot guarantee the correctness of the predicted types. Their performance significantly depends on the quality of the training data (i.e., DL models perform poorly on some common types that rarely appear in the training dataset). It is interesting to note that the static and DL-based approaches offer complementary benefits. Unfortunately, to our knowledge, precise type inference based on both static inference and neural predictions has not been exploited and remains an open challenge. In particular, it is hard to integrate DL models into the framework of rule-based static approaches. This paper fills the gap and proposes a hybrid type inference approach named HiTyper based on both static inference and deep learning. Specifically, our key insight is to record type dependencies among variables in each function and encode the dependency information in type dependency graphs (TDGs). Based on TDGs, we can easily integrate type inference rules in the nodes to conduct static inference and type rejection rules to inspect the correctness of neural predictions. HiTyper iteratively conducts static inference and DL-based prediction until the TDG is fully inferred. Experiments on two benchmark datasets show that HiTyper outperforms state-of-the-art DL models by exactly matching 10% more human annotations. HiTyper also achieves an increase of more than 30% on inferring rare types. Considering only the static part of HiTyper, it infers 2x ~ 3x more types than existing static type inference tools.

==> algs/importanalysis.tex <==
\begin{figure}[htb]
\centering
  \begin{minipage}{1.0\linewidth}
    \begin{algorithm}[H]
    \caption{Import Analysis}
    \label{alg:usertype}
    \begin{algorithmic}[1]
    \REQUIRE
    The given source code file set, $S$;
    % $srcfile$; 
    \\
    \ENSURE
    User-defined type set, $U$;
    % $usertype$;
    overloading user-defined type set, $O$;
    % $overloading\_usertype$;
    \STATE $U \leftarrow S$.classes
    % \STATE $fileset \leftarrow srcfile$
    \FORALL{$s \in S$}
    \FORALL{$i \in s$.imports}
    \IF{$i$ is class}
    \IF{hasOverloadingMethod($U$)}
    \STATE $O \leftarrow O \vee U$
    % $overloading\_usertype \leftarrow overloading\_usertype \vee u$
    \ENDIF
    \STATE $U \leftarrow U \vee i$
    % $usertype \leftarrow usertype \vee i$
    \ELSE
    \STATE $S \leftarrow$ $S \vee$ resolveFile($i$)
    \ENDIF
    \ENDFOR
    \ENDFOR
    \end{algorithmic}
    \end{algorithm}
\end{minipage}
\end{figure}

==> rules/typerejrule.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[t]{0.45\textwidth}
    \begin{align*}
    
    \end{align*}
    \end{minipage}
    \begin{minipage}[t]{0.45\textwidth}
    \begin{align*}
    
    \end{align*}
    \end{minipage}
\caption{Type rejection rules of expressions in Python}
\label{fig:typerejrule}
\end{figure*}

==> sections/rules.tex <==
\section{Rules}




\subsection{Typing Rules}










    


==> sections/setup.tex <==
\input{tables/testset}

\section{Implementation Details}\label{sec:setup}

\textbf{Dataset.}
We used the two Python datasets mentioned in Sec.~\ref{sec:motivation} for evaluation. One is the \textit{Typilus's Dataset} released by Allamanis \etal~\cite{typilus}; and the other one is \textit{ManyTypes4Py} released by A. M. Mir \etal~\cite{type4pydataset}, with the number of different types in the test set and more detailed statistics shown in Table~\ref{tab:testset} and Sec.~\ref{sec:motivation}, respectively.
% We have introduced the details of these two datasets in Sec.~\ref{sec:motivation}. Table~\ref{tab:testset} shows the number of different types in the test set we use. 


\textbf{Evaluation Metrics.}
Following the previous work~\cite{typilus,mir2021type4py}, we choose two metrics \textit{Exact Match} and \textit{Match to Parametric} for evaluation. The two metrics compute the ratio of results that: 1) \textit{Exact Match}: completely matches human annotations. 2) \textit{Match to Parametric}: satisfy exact match when ignoring all the type parameters. For example, \texttt{List[int]} and \texttt{List[str]} are considered as matched under this metric.
% measure the type inference results by computing the ratio of results that satisfy: 1) \textit{Exact Match}: completely matches human annotations. 2) \textit{Match to Parametric}: Exact match when ignoring the all type parameters. For example, \texttt{List[int]} and \texttt{List[str]} are considered as matched under this metric.

\textbf{Baseline Approaches.}
To verify the effectiveness of the proposed \tool, we choose 5 baseline approaches for comparison:

1) A naive baseline. It represents a basic data-driven method. We build this baseline following the work~\cite{typewriter}, which makes predictions by sampling form the distribution of the most frequent ten types.
% considers the ten most frequent types in the dataset and makes predictions by sampling from the distribution of the ten types. 
% This method is a simple data-driven method that does not consider code semantics or structure information.

2) \pytype~\cite{pytype} and \pyre~\cite{pyre}. They are two popular
% widely-used 
Python static type inference tools from Google and Facebook, respectively. 

3) \typilus~\cite{typilus} and Type4Py~\cite{mir2021type4py}. 
% They are DL models. 
\typilus utilizes code structural information, 
% by converting source code into graph with various edges
and is the first DL model with search-based validation.
% open type vocabulary \revise{[add validation?]}. 
Type4Py is the SOTA model which uses type clusters and hierarchical neural network.
% \typilus is a DL model which utilizes code structural information by converting source code into a graph with different kinds of edges. It is also the first DL model with open type vocabulary in this task. Type4Py is the SOTA model that uses type clusters and a hierarchical neural network to better capture the similarity between programs. 



\textbf{Implementation of \tool.}
\tool is implemented using Python with more than 9,000 lines of code.
% All the typing rules and rejection rules are designed based on Python's official documentation~\cite{py3doc} and its implementation CPython~\cite{cpython}. 
We use the Skip-Gram method~\cite{DBLP:conf/nips/MikolovSCCD13} to train the Word2Vec model in Sec.~\ref{sec:typereco} based on all the class names and variable names. The dimension of the word embeddings and window size are set as 256 and 10, respectively.

% The entire framework of \tool is implemented using Python, which contains more than 9,000 lines of code. We obtain all typing rules and rejection rules from Python's official documentation~\cite{py3doc} and its implementation CPython\footnote{https://github.com/python/cpython}. We use Word2Vec model from the gensim library~\cite{gensim} as the embedding when calculating the similarity between two types. We train the Word2Vec model by utilizing all the class names and variable names in the training set of \typilus. The dimension of the word embeddings and size of the context window are set as 256 and 10, respectively. Due to the small training corpus for Word2Vec, we choose Skip-Gram algorithm for model training~\cite{DBLP:conf/nips/MikolovSCCD13}. 




==> tables/ablation.tex <==
\begin{table*}[t]
    \centering
    \caption{Ablations of \tool when removing its component or changing its type matching methods (F1 Score)}
    \scalebox{0.88}{\begin{tabular}{lccc|ccc|ccc}
    \toprule
        \multirow{2}*{\textbf{Ablation}} & \multicolumn{3}{c}{\textbf{Argument}} & \multicolumn{3}{c}{\textbf{Return Value}} & \multicolumn{3}{c}{\textbf{User Defined}} \\
        \cmidrule{2-10}
        & Top-1 &Top-3 & Top-5 & Top-1 &Top-3 & Top-5 & Top-1 & Top-3 & Top-5  \\
       \midrule
        \textbf{Only Static Inference (No DL models)} & 0.13 & - & - & 0.52 & - & - & 0.08 & - & - \\
        \midrule
        \textbf{No Type Rejection} & 0.63 & 0.72 & 0.74 & 0.60 & 0.65 & 0.66 & 0.48 & 0.56 & 0.60 \\
        \midrule
        \midrule
        \textbf{No Type Correction} & 0.60 & 0.68 & 0.70 & 0.57 & 0.61 & 0.62 & 0.39 & 0.46 & 0.47 \\
        \midrule
        \textbf{Type Correction - Only Variable Names} & 0.57 & 0.64 & 0.64 & 0.58 & 0.63 & 0.65 & 0.35 & 0.39 & 0.40 \\
        \midrule
        \textbf{Type Correction - Only DL models} & 0.62 & 0.69 & 0.72 & 0.58 & 0.63 & 0.64 & 0.43 & 0.50 & 0.53 \\
        \midrule
        \midrule
        \textbf{Overall Framework} & 0.63 & 0.71 & 0.74 & 0.60 & 0.65 & 0.66 & 0.47 & 0.55 & 0.59 \\
        
        \bottomrule
    \end{tabular}
    }
    
    \label{tab:ablation}
\end{table*}

==> tables/annotation.tex <==
\begin{table}[htb]
    \centering
    \caption{Comparison of annotations inferred by \tool and \typilus}
    \scalebox{0.85}{\begin{tabular}{lccc}
    \toprule
         & \textbf{Top-1} & \textbf{Top-3} & \textbf{Top -5} \\
    \midrule
    \textbf{Total type slots} & 20,456 & 20,456 & 20456 \\
    \textbf{correctly inferred by \tool Only} & 2,313 & 2,363 & 2,390 \\
    \textbf{correctly inferred by \typilus Only} & 784 & 1,119 & 1,088 \\
    \textbf{correctly inferred by both tools} & 10,137 & 11,516 & 11,945 \\
    \textbf{Failed to infer by both tools} & 7,222 & 5,458 & 5,033 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:annotation}
\end{table}

==> tables/operation.tex <==
\begin{table}[htb]
    \centering
    \caption{Three kinds of operations}
    \scalebox{0.72}{\begin{tabular}{lccc}
    \toprule
        & \textbf{Unary Op} & \textbf{N-ary Op} & \textbf{Function Call} \\
    \midrule
         \textbf{Input} & x & x1,x2,... & arg1,arg2,... \\
    \midrule
         \textbf{Output} & z & z & z \\
    \midrule
    \textbf{Example} & z = not x & z = x1 + x2 & z = func(arg1, arg2) \\
    \midrule
    \multirow{2}*{\tabincell{l}{\textbf{Typing} \\ \textbf{Rule}}} & \multirow{2}*{$T_z \leftarrow \phi(T_x \backslash RT_x)$} & \multirow{2}*{\tabincell{c}{$T_z \leftarrow \phi_o(T_{x1} \backslash RT_{x1},...,$ \\ $T_{xn} \backslash RT_{xn} )$}} & \multirow{2}*{$T_z \leftarrow \phi_o(F, U, sig)$}\\
    & & & \\
    \midrule
    \multirow{5}*{\tabincell{l}{\textbf{Rejection} \\ \textbf{Rule}}} & \multirow{4}*{$RT_x \leftarrow R_o$} & \multirow{5}*{\tabincell{c}{$RL \leftarrow T_{x1} \times ... \times T_{xi} \times ...\times T_{xn}$ \\ $RL_t \leftarrow T_{x1} \times ... \times T_{xi}\backslash\{t\}$ \\ $\times ...\times T_{xn}$ \\ $RT_{xi} \leftarrow R_o \bigcup \{t | \forall t \in T_{xi},$ \\ $RL_t\in RL_o , RL \notin RL_o \}$}} & \multirow{5}*{$RT_{argi} \leftarrow \{\}$} \\
    & & & \\
    & & & \\
    & & & \\
    & & & \\
    \bottomrule
    \end{tabular}}
    \label{tab:operation}
\end{table}

==> tables/rej.tex <==
\begin{table}[htb]
    \centering
    \caption{Comparison on average number of annotations added per type slot by \tool and \typilus}
    \scalebox{0.9}{\begin{tabular}{lcccc}
    \toprule
         &  \multicolumn{2}{c}{\textbf{Argument}} & \multicolumn{2}{c}{\textbf{Return Value}}\\
    \midrule
         & Top-3 & Top-5 & Top-3 & Top-5 \\
    \midrule
    \textbf{\tool} & 1.99 & 2.42 & 1.82 & 2.22 \\
    \textbf{\typilus} & 2.62 & 3.63 & 2.98 & 4.49 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:rej}
\end{table}
